Towards Trustworthy Knowledge Graph Reasoning: An Uncertainty Aware Perspective

Recently, Knowledge Graphs (KGs) have been successfully coupled with Large Language Models (LLMs) to mitigate their hallucinations and enhance their reasoning capability, such as in KG-based retrieval-augmented frameworks. However, current KG-LLM frameworks lack rigorous uncertainty estimation, limiting their reliable deployment in high-stakes applications. Directly incorporating uncertainty quantification into KG-LLM frameworks presents challenges due to their complex architectures and the intricate interactions between the knowledge graph and language model components. To address this gap, we propose a new trustworthy KG-LLM framework, Uncertainty Aware Knowledge-Graph Reasoning (UAG), which incorporates uncertainty quantification into the KG-LLM framework. We design an uncertainty-aware multi-step reasoning framework that leverages conformal prediction to provide a theoretical guarantee on the prediction set. To manage the error rate of the multi-step process, we additionally introduce an error rate control module to adjust the error rate within the individual components. Extensive experiments show that our proposed UAG can achieve any pre-defined coverage rate while reducing the prediction set/interval size by 40% on average over the baselines.

==> AnonymousSubmission/LaTeX/sections/checklist.tex <==
%to be updated, just copied from another paper with their answers below

\newpage
\section{Reproducibility Checklist
}
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) Yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) Yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) Yes

\end{itemize}

Does this paper make theoretical contributions? (yes/no) Yes

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. yes
    \item All novel claims are stated formally (e.g., in theorem statements). yes 
    \item Proofs of all novel claims are included. yes
    \item Proof sketches or intuitions are given for complex and/or novel results. yes 
    \item Appropriate citations to theoretical tools used are given. yes
    \item All theoretical claims are demonstrated empirically to hold. partial
    \item All experimental code used to eliminate or disprove claims is included. yes 
\end{itemize}

Does this paper rely on one or more datasets? (yes/no) Yes 

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) Yes
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) NA, we use publicly available dataset.
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) NA, we use publicly available dataset.
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) Yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) Yes
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) NA
\end{itemize}

Does this paper include computational experiments? (yes/no) Yes

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no). Yes
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) Partial, since some of the results reported in this paper were taken from prior work that utilized the same dataset splits without publicly available code
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) Partial, since some of the results reported in this paper were taken from prior work that utilized the same dataset splits without publicly available code
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) Yes
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) Yes
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) Yes
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) Yes
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) no
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) Yes
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) No
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) Yes
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) yes
\end{itemize}

